Gluing equations for PGL(n,C)-representations of 3-manifolds

In a previous paper, we parametrized boundary-unipotent representations of a 3-manifold group into SL(n,C) using Ptolemy coordinates, which were inspired by A-coordinates on higher Teichm\"uller space due to Fock and Goncharov. In this paper, we parametrize representations into PGL(n,C) using shape coordinates which are a 3-dimensional analogue of Fock and Goncharov's X-coordinates. These coordinates satisfy equations generalizing Thurston's gluing equations. These equations are of Neumann-Zagier type and satisfy symplectic relations with applications in quantum topology. We also explore a duality between the Ptolemy coordinates and the shape coordinates.

==> figures_gen/Figure8Sister.tex <==
\begingroup
 \setlength{\unitlength}{0.8pt}
 \begin{picture}(522.58881,212.78915)
 \put(0,0){\includegraphics{figures_gen/Figure8Sister_included}}
 \end{picture}
\endgroup


==> figures_gen/Figure8ordered.tex <==
\begingroup
 \setlength{\unitlength}{0.8pt}
 \begin{picture}(521.26776,212.78915)
 \put(0,0){\includegraphics{figures_gen/Figure8ordered_included}}
 \end{picture}
\endgroup


==> figures_gen/LocalModelEdgeGluing.tex <==
\begingroup
 \setlength{\unitlength}{0.8pt}
 \begin{picture}(167.0246,196.7498)
 \put(0,0){\includegraphics{figures_gen/LocalModelEdgeGluing_included}}
 \end{picture}
\endgroup


==> figures_gen/LocalModelFaceGluing.tex <==
\begingroup
 \setlength{\unitlength}{0.8pt}
 \begin{picture}(206.95085,252.85754)
 \put(0,0){\includegraphics{figures_gen/LocalModelFaceGluing_included}}
 \end{picture}
\endgroup


==> figures_gen/PtolemyCoordinatesOnSimplex.tex <==
\begingroup
 \setlength{\unitlength}{0.8pt}
 \begin{picture}(225.86356,182.21802)
 \put(0,0){\includegraphics{figures_gen/PtolemyCoordinatesOnSimplex_included}}
 \end{picture}
\endgroup


==> figures_gen/SubSimplices.tex <==
\begingroup
 \setlength{\unitlength}{0.8pt}
 \begin{picture}(273.73523,206.15857)
 \put(0,0){\includegraphics{figures_gen/SubSimplices_included}}
 \end{picture}
\endgroup


==> figures_gen/tetGluing1.tex <==
\begingroup
 \setlength{\unitlength}{0.8pt}
 \begin{picture}(581.89203,534.09308)
 \put(0,0){\includegraphics{figures_gen/tetGluing1_included}}
 \end{picture}
\endgroup


==> figures_gen/tetInternalGluingEquation.tex <==
\begingroup
 \setlength{\unitlength}{0.8pt}
 \begin{picture}(848.67828,539.34344)
 \put(0,0){\includegraphics{figures_gen/tetInternalGluingEquation_included}}
 \end{picture}
\endgroup


==> mathdots.tex <==
%%
%% This is file `mathdots.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% mathdots.dtx  (with options: `tex')
%% 
%% -------------------------------------------------------------------
%% 
%% Copyright 2001--2006, Daniel H. Luecking
%% 
%% Mathdots may be distributed and/or modified under the conditions of the
%% LaTeX Project Public License, either version 1.3 of this license or (at
%% your option) any later version. The latest version of this license is in
%%    <http://www.latex-project.org/lppl.txt>
%% and version 1.3 or later is part of all distributions of LaTeX version
%% 2003/12/01 or later.
%% 
%% Mathdots has maintenance status "author-maintained". The Current
%% Maintainer is Daniel H. Luecking. The Base Interpreters associated with
%% mathdots are plain TeX and LaTeX
%% 
\def\mathdotsfiledate{2006/03/16}%
\def\mathdotsfileversion{0.8}%
\expandafter
\ifx\csname MathDots\mathdotsfileversion\endcsname\relax
\else
  \immediate\write16{Mathdots already loaded.}\expandafter\endinput
\fi
\immediate\write16{Package mathdots, \mathdotsfiledate\space version
  \mathdotsfileversion.}%
\expandafter\edef\csname MathDots\mathdotsfileversion\endcsname{%
    \catcode`\noexpand\@=\the\catcode`@}%
\catcode`\@=11
\def\@nameuse#1{\csname#1\endcsname}%
\def\MD@us#1{\@nameuse{#1style}}%
\def\MD@uf#1{\@nameuse{#1font}0}%
\def\MD@t{text}\def\MD@s{script}\def\MD@ss{scriptscript}%
\newdimen\MD@unit \MD@unit\p@
\def\MD@changestyle#1{\relax\MD@unit0.1\fontdimen6\MD@uf{#1}%
  \everymath\expandafter{\the\everymath\MD@us{#1}}}%
\def\MD@dot{$\m@th\ldotp$}%
\def\MD@palette#1{\mathchoice{#1\MD@t}{#1\MD@t}{#1\MD@s}{#1\MD@ss}}%
\def\MD@ddots#1{{\MD@changestyle{#1}%
  \mkern1mu\raise7\MD@unit\vbox{\kern7\MD@unit\hbox{\MD@dot}}%
  \mkern2mu\raise4\MD@unit\hbox{\MD@dot}%
  \mkern2mu\raise \MD@unit\hbox{\MD@dot}\mkern1mu}}%
\def\MD@vdots#1{\vbox{\MD@changestyle{#1}%
  \baselineskip4\MD@unit\lineskiplimit\z@
  \kern6\MD@unit\hbox{\MD@dot}\hbox{\MD@dot}\hbox{\MD@dot}}}%
\def\MD@iddots#1{{\MD@changestyle{#1}%
  \mkern1mu\raise \MD@unit\hbox{\MD@dot}%
  \mkern2mu\raise4\MD@unit\hbox{\MD@dot}%
  \mkern2mu\raise7\MD@unit\vbox{\kern7\MD@unit\hbox{\MD@dot}}}}%
\def\fixedvdots{%
  \vbox{\baselineskip4\p@ \lineskiplimit\z@
  \kern6\p@\hbox{.}\hbox{.}\hbox{.}}}%
\def\fixedddots{%
  \mathinner{\mkern1mu
  \raise7\p@\vbox{\kern7\p@\hbox{.}}\mkern2mu
  \raise4\p@\hbox{.}\mkern2mu
  \raise\p@\hbox{.}\mkern1mu}}%
\def\fixediddots{%
  \mathinner{\mkern1mu
  \raise\p@\hbox{.}\mkern2mu
  \raise4\p@\hbox{.}\mkern2mu
  \raise7\p@\vbox{\kern7\p@\hbox{.}}\mkern1mu}}%
\let\originalddots=\ddots
\let\originalvdots=\vdots
\let\originaliddots=\iddots
\def\ddots{%
  \mathinner{\MD@palette\MD@ddots}}%
\def\iddots{%
  \mathinner{\MD@palette\MD@iddots}}%
\def\vdots{%
  \mathinner{\MD@palette\MD@vdots}}%
\wlog{Mathdots Info: Redefining \string\ddots.}%
\wlog{Mathdots Info: Redefining \string\vdots.}%
\newbox\MD@dotsbox
\newmuskip\MD@prekern
\newmuskip\MD@postkern
\newmuskip\MD@dotkern
\MD@prekern 0mu
\MD@postkern -1mu
\MD@dotkern -1.3mu
\def\MD@dotsaccent#1{\mathpalette{\MD@@dotsaccent{#1}}}%
\def\MD@@dotsaccent#1#2#3{%
  {\setbox\MD@dotsbox\hbox{$#2\mkern\MD@prekern#1\mkern\MD@postkern$}%
   \mathop{#3\kern\z@}\limits^{%
   \text{\vbox to-1.4\ex@{\kern-1.8\ex@\copy\MD@dotsbox\vss}}}}%
}%
\let\originaldddot \dddot
\let\originalddddot\ddddot
\def\amstexfmtname{AmS-TeX}%
\ifx\amstexfmtname\fmtname
  \def\MD@D{\mathchar"5F\mkern\MD@dotkern}%
  \wlog{Mathdots Info: Redefining \string\dddot.}%
  \wlog{Mathdots Info: Redefining \string\ddddot.}%
  \def\dddot {\MD@dotsaccent{\MD@D\MD@D\MD@D}}%
  \def\ddddot{\MD@dotsaccent{\MD@D\MD@D\MD@D\MD@D}}%
\fi
\csname MathDots\mathdotsfileversion\endcsname
\endinput
%%
%% End of file `mathdots.tex'.


==> mathdots_README <==

This is the mathdots package, version 0.8.

This package changes the basic LaTeX and plain TeX commands \ddots and
\vdots so that they properly change size when font sizes change, and
when they are used in superscripts and subscripts. It also adds the
command \iddots ()for inverse diagonal dots) which slants the opposite
way from \ddots.

In addition, if it detects AMSLaTeX (or AMSTeX in plain TeX) it defines
improved versions of the \dddot and \ddddot commands that place three
and four dots on a math symbol (similar to the math accent commands \dot
and \ddot). These also are arranged to change size correctly and some
placement bugs are corrected.

Other (minor) improvements: the commands \vdots, \ddots and \iddots
select the dot from the math fonts instead of the text fonts, so they
always match math punctuation dots. The \dddot and \ddddot commands
select the accent dot (same one placed by \dot).

File list:

mathdots.dtx    The code
mathdots.pdf    The manual
mathdots.ins    unpacking script
mdtest.tex      Test file
README          This file

Installation:

Run tex or latex on mathdots.ins to unpack the files. Copy mathdots.tex
where tex will find it and mathdots.sty where latex will find it. Copy
the remaining files to your documentation area.

Daniel H. Luecking, \luecking \at \uark \dot \edu


